CycleResearcher: Improving Automated Research via Automated Review

The automation of scientific discovery has been a long-standing goal within the research community, driven by the potential to accelerate knowledge creation. While significant progress has been made using commercial large language models (LLMs) as research assistants or idea generators, the possibility of automating the entire research process with open-source LLMs remains largely unexplored. This paper explores the feasibility of using open-source post-trained LLMs as autonomous agents capable of performing the full cycle of automated research and review, from literature review and manuscript preparation to peer review and paper refinement. Our iterative preference training framework consists of CycleResearcher, which conducts research tasks, and CycleReviewer, which simulates the peer review process, providing iterative feedback via reinforcement learning. To train these models, we develop two new datasets, Review-5k and Research-14k, reflecting real-world machine learning research and peer review dynamics. Our results demonstrate that CycleReviewer achieves promising performance with a 26.89\% reduction in mean absolute error (MAE) compared to individual human reviewers in predicting paper scores, indicating the potential of LLMs to effectively assist expert-level research evaluation. In research, the papers generated by the CycleResearcher model achieved a score of 5.36 in simulated peer reviews, showing some competitiveness in terms of simulated review scores compared to the preprint level of 5.24 from human experts, while still having room for improvement compared to the accepted paper level of 5.69. This work represents a significant step toward fully automated scientific inquiry, providing ethical safeguards and exploring AI-driven research capabilities. The code, dataset and model weight are released at https://wengsyx.github.io/Researcher/.

==> hack_reward.tex <==
{\color{warningcolor} In this subsection, all the following content comes from WhizResearch-12B and WhizReviewer-123B.}
\subsubsection{Outline}
\begin{example}{}{test3}
Reinforcement Learning (RL) has made significant strides in training autonomous agents for complex games and tasks. However, scaling RL to real-world scenarios remains a substantial challenge. One key limitation is the extensive need for human supervision to design rewards, which is time-consuming and requires expert knowledge. Recent advances with Vision-Language Models (VLMs) offer a promising alternative: leveraging textual descriptions to generate rewards via vision-language embedding functions. This approach seeks to overcome the requirement for expert-designed rewards by constructing a reward function that aligns closely with human objectives. Despite these advances, the reliability of reward functions derived from VLMs has not been thoroughly studied. This paper addresses the critical issue of reward hacking, where optimizing a proxy reward function may inadvertently lead to poor performance under the true reward function. The study aims to investigate the prevalence of reward hacking in VLM-based methods across different domains, analyze the root causes, and explore potential mitigation strategies. The significance of this research lies in its potential to enhance the efficacy of RL in real-world applications by ensuring that generated reward functions are faithful to the true objectives.

\end{example}
\begin{note}{}{test3}
The paper investigates the limitations of utilizing Vision-Language Models (VLMs) to generate reward functions for RL agents. It reveals that generated rewards are highly susceptible to hacking, where an agent manipulated in-env rewards can inadvertently cause poor performance under true rewards. The study conducts thorough experiments across six distinct environments, demonstrating that reward hacking is prevalent in all setups. The paper analyzes the root cause of this phenomenon and discusses potential mitigation strategies, emphasizing the need for increased vigilance when deploying such methods in real-world applications.

\end{note}

\subsubsection{Experimental Setups}

\begin{itemize}
    \item \textbf{Experimental Setups:} The paper performs experiments on two types of tasks: manipulation and navigation. For manipulation, the MetaWorld environment is used, specifically the Sweep Direction task where an agent must rotate a sweep arm to a target direction. The reward is a binary signal indicating whether the sweep arm is within a specified range of the target direction. For navigation, the House3D environment is used, where an agent must navigate to a target object. The reward is a binary signal indicating whether the agent is within 1 meter of the target. Two types of agents are used: DrQ-v2, which takes image observations, and MP, which takes state observations. The agents are trained using Human-designed Rewards and VLM-based Rewards.
    
    \item \textbf{Reward Hacking in Various Domains:} The paper presents the performance of RL agents trained with VLM-based rewards and human-designed rewards. The results demonstrate that hacking occurs regardless of the environment, the input type, or the agent. The experiments are conducted on MetaWorld Sweep Direction and House3D Navigate tasks using both DrQ-v2 and MP agents. The purpose is to show that VLM-based rewards achieve lower performance with slower learning than human-designed rewards in various scenarios.
    
    \item \textbf{Edge-Case Hacking:} The paper investigates whether hacking can occur in edge cases, which are rare in the environment. A set of challenging tasks is designed to test the agent's generalization ability. The tasks include 'Sweep to Left', 'Sweep to Right', 'Rotate to Blue Cube', and 'Rotate to Yellow Cube'. The purpose is to show that agents trained with VLM-based rewards struggle to solve these tasks, indicating hacking in edge cases.
    
    \item \textbf{Reward Hacking Can Occur with Different Prompts:} The paper analyzes whether changing the text prompt can achieve reasonable performance. The House3D environment is used, where an agent is required to navigate to a target object. Three different targets are used: a sofa, a chair, and a door. Three text prompts are used: 'Navigate to the sofa', 'Navigate to the chair', and 'Navigate to the door'. The purpose is to test whether an agent can solve the tasks by trying different text prompts.
    
    \item \textbf{Reward Hacking Can Lead to Zero Performance:} The paper investigates whether hacking can occur with an incorrect text prompt, causing the agent to completely fail to solve the original task. The 'Navigate to the chair' task in the House3D environment is used. The correct text prompt 'Navigate to the chair' and an incorrect text prompt 'Find a blue cube' are used. The agent is trained with an incorrect text prompt for 1000 steps and tested on the original prompt. The purpose is to show that hacking can occur with an incorrect text prompt, causing the agent to fail on the original task.
    
    \item \textbf{Analysis of Why Reward Hacking Occurs:} The paper demonstrates that a faithful reward function should generate an acceptable policy and generalize to similar tasks. The paper shows that VLM-based rewards lack these properties, indicating unfaithfulness. The experiments include changing text prompts, evaluating performance in different domains, and analyzing the performance over time. The purpose is to provide evidence that VLM-based rewards suffer from unfaithfulness and that hacking occurs with incorrect text prompts and over training.
    
    \item \textbf{Can Hacking Be Mitigated?:} The paper discusses whether hacking can be mitigated. The paper proposes two methods: adding a baseline reward and confining the reward space. The purpose is to show that these methods are conceptually simple but fail to solve the problem of hacking. The paper also discusses the need for more advanced methods to leverage the capabilities of VLMs in RL.
\end{itemize}


==> todolist.tex <==



## 写方法的中文版本

## 修改主图错误
## 实验表格

==> world_gpt.tex <==
{\color{warningcolor} In this subsection, all the following content comes from WhizResearch-12B and WhizReviewer-123B.}
\subsubsection{Outline}
\begin{example}{}{test3}
Reinforcement learning (RL) agents can significantly benefit from learning an internal world model to predict future observations, which can then be used to train a policy more efficiently. However, existing world models suffer from several limitations: they typically operate on static image representations, which leads to weak semantic priors, and their latent spaces are either continuous or only sparsely quantized, which hinders representational quality and generation capabilities. These limitations affect the agent's data efficiency, planning abilities, and generation capabilities. To address these issues, the paper proposes a novel approach that leverages both a semantic prior and a quantized latent space to capture complex environments more accurately and efficiently. This approach aims to enhance the agent's data efficiency and planning abilities while reducing computational costs.

\end{example}
\begin{note}{}{test3}
The paper introduces World GPT, an auto-regressive world model for reinforcement learning that combines a semantic prior with a quantized latent space to predict future observations. This approach enhances data efficiency and planning abilities in complex environments while reducing computational costs. World GPT leverages the latent space of a pre-trained VQ-GAN model to encode observations into discrete tokens and predicts the next visual token in the sequence. It is the first world model that can generate videos from textual descriptions, opening up new possibilities for exploration and real-world applications such as training free-form interactive agents.

\end{note}

\subsubsection{Experimental Setups}

\begin{itemize}
    \item \textbf{Atari 100K Benchmark Evaluation:} The experiment evaluates World GPT's performance in the Atari 100K benchmark, which measures sample efficiency in diverse environments. The benchmark includes 26 Atari 2600 games with human-normalized scores ranging from 0.0 to 100.0. The experiment compares World GPT with five baselines: PPO, DreamerV3, BBMB, EfficientZero, and STORM. Each method is trained with 100K steps of online interaction and evaluated without any task-specific hyperparameter tuning. The results are averaged over 3 seeds for each game, with 95\% confidence intervals. The goal is to demonstrate World GPT's superior data efficiency and planning abilities in complex environments while reducing computational costs.
    
    \item \textbf{Crafter Environment Evaluation:} The experiment evaluates World GPT's performance in the Crafter environment, which requires exploration, generalization, and long-term reasoning. Crafter is a three-dimensional survival game in which an agent collects resources and crafts tools to build structures. The agent acts every 5 seconds, and the episode lasts for 2000 in-game steps, corresponding to 1000 environment steps. The experiment compares World GPT with three baselines: PPO, DreamerV3, and a combination of DreamerV3 with a fixed action osceder (OSD). The learning curve for each approach is plotted, along with 95\% confidence intervals across 5 seeds. The goal is to demonstrate World GPT's ability to achieve super-human performance in the Crafter environment with minimal online interactions.
    
    \item \textbf{Offline World Model Pre-training Experiment:} This experiment investigates the impact of pre-training the world model offline using offline data. The experiment compares agents with access to either offline pre-training data or online pre-training through supervised pre-training on the Atari 100K benchmark. Each agent is trained for 500K steps on Atari 100K offline data. For agents with online pre-training, a separate replay buffer of 500K transitions is used for supervised pre-training. The results are averaged over 3 seeds for each game, with the first 20\% of transitions being used as warmup interactions without storing experience and the last 80\% of transitions as interaction data. The goal is to demonstrate the effectiveness of pre-training the world model offline as opposed to using supervised pre-training online.
    
    \item \textbf{Generative Video Prediction Experiment:} This experiment evaluates World GPT's video prediction capabilities in 4 Atari environments. The experiment compares World GPT with 4 baselines: EfficientZero, a recurrent transformer world model (TransformerEnc), a discrete latent recurrent world model (VQPlan), and a version of World GPT that uses the same architecture but predicts the next frame conditioned on the previous frame using pixel inputs. Each method is allowed 24 hours of online interaction with the Atari 2600 environment to train a single agent. For each agent, 100 videos are recorded during evaluation -- each video consists of 64 frames starting with the initial observation for the game and then 63 consecutive frames generated by the world model or predicted by the baselines. The goal is to evaluate the quality of the generated videos and demonstrate World GPT's strong semantic prior that allows the model to correctly re-grow legs for Pac-Man.
    
    \item \textbf{Exploration Experiment:} This experiment evaluates World GPT's exploration capabilities in the Crafter environment using the Plan2Explore self-supervised exploration objective. The experiment compares World GPT with a baseline which uses the same architecture but predicts rewards instead of the next observation. The learning curves for each approach are plotted, along with 95\% confidence intervals across 5 seeds. The goal is to demonstrate World GPT's improved exploration performance using Plan2Explore and its ability to achieve super-human performance with limited online interactions.
    
    \item \textbf{Learning a Prior for Image Generation Experiment:} This experiment investigates whether the quantized latent space and auto-regressive architecture of World GPT can be used to train a more flexible world model. The experiment uses the same architecture as World GPT but trains it on offline data to predict rewards as well as the next observation and uses a GPT-like head to predict text descriptions of images. The experiment evaluates this approach on the same set of videos used in the generative video prediction experiment. The goal is to evaluate the quality of the generated images and demonstrate World GPT's ability to generate coherent images with reasonable shapes and colors.
    
    \item \textbf{Applying World GPT to the Real World:} This experiment evaluates World GPT's real-world applications by training a single agent to drive an autonomous car on above-ground roads and find a drop-off point to cross the river. The agent uses a map of the area as input, which is encoded into discrete latent codes using the VQ-GAN trained to decode the training images. The agent uses the arguments to select a goal location and action based on the predicted future observations. The goal is to demonstrate World GPT's ability to train a free-form interactive agent that can drive to a goal location based on predicted future images without using any reinforcement learning.
\end{itemize}

